A Search Worth a Billion Pixels: Explaining Gigapixel Classifiers

Perturbation-based attribution methods explain model predictions without accessing their internal representations, but scaling them to high-resolution images requires balancing perturbation granularity and computational cost. Fine-grained perturbations require many model evaluations, whereas coarse masks may overlook small but relevant evidence. We introduce Wavelet Find-and-Refine (WaFR), a model-agnostic attribution method combining adaptive hierarchical search with sparse multiscale regression. By selectively refining regions that influence the prediction, WaFR maintains fine-grained localisation with a computational cost that depends on the spatial distribution of the evidence. As image resolution increases to 8,192 pixels per side, WaFR maintains a Pointing Game score of at least .995 in controlled localisation experiments, including at matched forward-pass budgets. On gigapixel whole-slide images, it requires a median of 176 forward passes and achieves the highest mean patch-level AUROC among the evaluated perturbation-based methods (.949).

==> tables/A5a_full_rows_487.tex <==
\addlinespace[2pt]
\tabgroup{11}{Methods marked \sa, on all 1,000 images}
RISE & .130\ci{.010} & .736\ci{.015} & .382\ci{.014} & \na & \na & .115\ci{.009} & .675\ci{.015} & .386\ci{.014} & \na & \na \\
LIME & .134\ci{.008} & .718\ci{.016} & .391\ci{.011} & \na & \na & .111\ci{.007} & .635\ci{.016} & .388\ci{.013} & \na & \na \\
PartitionSHAP & .066\ci{.005} & .734\ci{.015} & .494\ci{.012} & \na & \na & .051\ci{.004} & .659\ci{.016} & .533\ci{.012} & \na & \na \\
Sobol & .111\ci{.008} & .667\ci{.018} & .455\ci{.014} & \na & \na & .097\ci{.007} & .582\ci{.019} & .477\ci{.014} & \na & \na \\
LIMA & .141\ci{.009} & .675\ci{.016} & .256\ci{.012} & \na & \na & .115\ci{.008} & .605\ci{.018} & .287\ci{.013} & \na & \na \\
MoXI & .315\ci{.014} & .564\ci{.020} & -.050\ci{.012} & \na & \na & .220\ci{.012} & .508\ci{.018} & .032\ci{.012} & \na & \na \\
WCAM & .182\ci{.011} & .649\ci{.019} & .316\ci{.014} & \na & \na & .167\ci{.010} & .573\ci{.018} & .317\ci{.014} & \na & \na \\


==> tables/A5a_imagenet_cnn_body.tex <==
\tabgroup{11}{References}
\ctrl{Random map} & \ctrl{.152\ci{.009}} & \ctrl{.352\ci{.016}} & \ctrl{-.050\ci{.008}} & \ctrl{.385\ci{.061}} & \ctrl{.391\ci{.032}} & \ctrl{.090\ci{.007}} & \ctrl{.238\ci{.012}} & \ctrl{-.043\ci{.008}} & \ctrl{.385\ci{.061}} & \ctrl{.391\ci{.032}} \\
\ctrl{Centre map} & \ctrl{.193\ci{.011}} & \ctrl{.577\ci{.018}} & \ctrl{.184\ci{.015}} & \ctrl{.692\ci{.057}} & \ctrl{.500\ci{.037}} & \ctrl{.169\ci{.010}} & \ctrl{.507\ci{.020}} & \ctrl{.172\ci{.014}} & \ctrl{.692\ci{.057}} & \ctrl{.500\ci{.037}} \\
\addlinespace[2pt]
\tabgroup{11}{Gradient- and activation-based}
Saliency & .126\ci{.009}\sig & .467\ci{.017}\sig & .228\ci{.015}\sig & .603\ci{.061}\sig & .474\ci{.033}\sig & .077\ci{.007}\sig & .371\ci{.015}\sig & .305\ci{.018}\sig & .692\ci{.057}\sig & .491\ci{.031}\sig \\
Integrated Gradients & .142\ci{.010}\sig & .381\ci{.018}\sig & .080\ci{.009}\sig & .615\ci{.065}\sig & .500\ci{.032}\sig & .093\ci{.008} & .265\ci{.015}\sig & .119\ci{.010}\sig & .725\ci{.057}\sig & .529\ci{.033}\sig \\
SmoothGrad & .098\ci{.007}\sig & .626\ci{.017}\sig & .373\ci{.017}\sig & .757\ci{.035}\sig & .600\ci{.034}\sig & .068\ci{.005}\sig & .529\ci{.018}\sig & .377\ci{.016}\sig & .720\ci{.034}\sig & .568\ci{.032}\sig \\
Grad-CAM & .153\ci{.009} & .685\ci{.016}\sig & .384\ci{.012}\sig & .800\ci{.050}\sig & .522\ci{.032}\sig & .109\ci{.008} & .611\ci{.018}\sig & .430\ci{.013}\sig & .795\ci{.050}\sig & .531\ci{.030}\sig \\
Grad-CAM++ & .156\ci{.010} & .672\ci{.017}\sig & .360\ci{.014}\sig & .806\ci{.049}\sig & .486\ci{.031}\sig & .113\ci{.008} & .582\ci{.018}\sig & .435\ci{.013}\sig & .834\ci{.045}\sig & .526\ci{.031}\sig \\
\addlinespace[2pt]
\tabgroup{11}{Perturbation-based}
Occlusion & .192\ci{.015} & .655\ci{.017}\sig & .310\ci{.020}\sig & .718\ci{.043}\sig & .520\ci{.036}\sig & .107\ci{.008} & .615\ci{.017}\sig & .440\ci{.014}\sig & .743\ci{.039}\sig & .528\ci{.032}\sig \\
RISE\sa & .125\ci{.019} & \best{.735}\ci{.030}\sig & .393\ci{.029}\sig & .803\ci{.115}\sig & .398\ci{.063}\sig & .111\ci{.018} & \best{.673}\ci{.033}\sig & .401\ci{.029}\sig & \second{.869}\ci{.082}\sig & .398\ci{.064}\sig \\
LIME\sa & .132\ci{.017} & .714\ci{.034}\sig & .403\ci{.023}\sig & .773\ci{.079}\sig & .629\ci{.059}\sig & .108\ci{.016} & .639\ci{.033}\sig & .406\ci{.021}\sig & .802\ci{.082}\sig & .611\ci{.063}\sig \\
KernelSHAP & .142\ci{.010} & .645\ci{.018}\sig & .397\ci{.015}\sig & .799\ci{.045}\sig & \best{.679}\ci{.033}\sig & .117\ci{.009} & .556\ci{.019}\sig & .386\ci{.018}\sig & .760\ci{.048}\sig & .655\ci{.034}\sig \\
PartitionSHAP\sa & \best{.063}\ci{.010}\sig & \second{.728}\ci{.032}\sig & \second{.496}\ci{.025}\sig & .824\ci{.089}\sig & \second{.667}\ci{.053}\sig & \second{.052}\ci{.009}\sig & \second{.656}\ci{.032}\sig & \second{.539}\ci{.023}\sig & .821\ci{.088}\sig & \second{.664}\ci{.052}\sig \\
h-Shap & .332\ci{.014} & .513\ci{.019}\sig & .118\ci{.015}\sig & .705\ci{.047}\sig & .666\ci{.053}\sig & .266\ci{.014} & .433\ci{.018}\sig & .159\ci{.015}\sig & .745\ci{.047}\sig & \best{.737}\ci{.047}\sig \\
ShapBPT & .125\ci{.008}\sig & .714\ci{.016}\sig & .435\ci{.015}\sig & \second{.826}\ci{.042}\sig & .637\ci{.030}\sig & .096\ci{.006} & .640\ci{.019}\sig & .457\ci{.015}\sig & .815\ci{.041}\sig & .639\ci{.030}\sig \\
Sobol\sa & .113\ci{.015}\sig & .660\ci{.037}\sig & .448\ci{.030}\sig & .787\ci{.099}\sig & .657\ci{.055}\sig & .097\ci{.013} & .576\ci{.039}\sig & .489\ci{.028}\sig & \best{.885}\ci{.082}\sig & .643\ci{.061}\sig \\
HSIC & .109\ci{.007}\sig & .674\ci{.017}\sig & .448\ci{.018}\sig & .814\ci{.049}\sig & .662\ci{.029}\sig & .100\ci{.007} & .604\ci{.019}\sig & .470\ci{.014}\sig & .794\ci{.057}\sig & .637\ci{.031}\sig \\
LIMA\sa & .144\ci{.018} & .664\ci{.034}\sig & .248\ci{.026}\sig & .698\ci{.101}\sig & .504\ci{.067}\sig & .108\ci{.014} & .607\ci{.034}\sig & .292\ci{.026}\sig & .704\ci{.102}\sig & .520\ci{.071}\sig \\
MoXI\sa & .314\ci{.028} & .550\ci{.039}\sig & -.035\ci{.025} & .405\ci{.115} & .363\ci{.065} & .212\ci{.023} & .500\ci{.038}\sig & .035\ci{.025}\sig & .362\ci{.122} & .385\ci{.066} \\
WCAM\sa & .185\ci{.023} & .648\ci{.036}\sig & .317\ci{.027}\sig & .754\ci{.115}\sig & .557\ci{.059}\sig & .173\ci{.021} & .579\ci{.037}\sig & .347\ci{.025}\sig & .623\ci{.131} & .528\ci{.061}\sig \\
\addlinespace[2pt]
\tabgroup{11}{Ours}
\ours{\method} & \second{.069}\ci{.006}\sig & .717\ci{.016}\sig & \best{.537}\ci{.012}\sig & \best{.846}\ci{.045}\sig & .606\ci{.027}\sig & \best{.049}\ci{.004}\sig & .640\ci{.017}\sig & \best{.570}\ci{.011}\sig & .850\ci{.045}\sig & .611\ci{.028}\sig \\


==> tables/A5b_imagenet_vit_body.tex <==
\tabgroup{11}{References}
\ctrl{Random map} & \ctrl{.302\ci{.013}} & \ctrl{.563\ci{.017}} & \ctrl{-.033\ci{.008}} & \ctrl{.385\ci{.061}} & \ctrl{.391\ci{.032}} & \ctrl{.330\ci{.013}} & \ctrl{.545\ci{.017}} & \ctrl{-.020\ci{.007}} & \ctrl{.385\ci{.061}} & \ctrl{.391\ci{.032}} \\
\ctrl{Centre map} & \ctrl{.327\ci{.013}} & \ctrl{.625\ci{.016}} & \ctrl{.112\ci{.012}} & \ctrl{.692\ci{.057}} & \ctrl{.500\ci{.037}} & \ctrl{.335\ci{.011}} & \ctrl{.614\ci{.015}} & \ctrl{.072\ci{.010}} & \ctrl{.692\ci{.057}} & \ctrl{.500\ci{.037}} \\
\addlinespace[2pt]
\tabgroup{11}{Gradient- and activation-based}
Saliency & .260\ci{.012}\sig & .592\ci{.015}\sig & .025\ci{.011}\sig & .348\ci{.069} & .395\ci{.034} & .279\ci{.012}\sig & .567\ci{.015}\sig & .007\ci{.009}\sig & .332\ci{.061} & .369\ci{.035} \\
Integrated Gradients & .210\ci{.011}\sig & .603\ci{.016}\sig & .057\ci{.009}\sig & .453\ci{.061} & .423\ci{.031}\sig & .237\ci{.010}\sig & .593\ci{.016}\sig & .021\ci{.007}\sig & .340\ci{.057} & .352\ci{.037} \\
SmoothGrad & .173\ci{.011}\sig & .651\ci{.015}\sig & .126\ci{.015}\sig & .616\ci{.040}\sig & .512\ci{.032}\sig & .196\ci{.011}\sig & .638\ci{.014}\sig & .051\ci{.013}\sig & .601\ci{.042}\sig & .491\ci{.032}\sig \\
Grad-CAM & .329\ci{.014} & .583\ci{.017}\sig & .042\ci{.014}\sig & .517\ci{.062}\sig & .451\ci{.042}\sig & .221\ci{.011}\sig & .635\ci{.015}\sig & .058\ci{.011}\sig & .850\ci{.045}\sig & .513\ci{.034}\sig \\
Grad-CAM++ & .368\ci{.014} & .564\ci{.019} & -.011\ci{.011}\sig & .377\ci{.061} & .352\ci{.044} & .324\ci{.012} & .582\ci{.015}\sig & .029\ci{.010}\sig & .443\ci{.067} & .437\ci{.036}\sig \\
\addlinespace[2pt]
\tabgroup{11}{Perturbation-based}
Occlusion & .300\ci{.013} & .676\ci{.014}\sig & .217\ci{.012}\sig & .537\ci{.050}\sig & .454\ci{.035}\sig & .396\ci{.016} & .656\ci{.014}\sig & .191\ci{.013}\sig & .594\ci{.049}\sig & .439\ci{.039}\sig \\
RISE\sa & .223\ci{.026}\sig & \best{.744}\ci{.022}\sig & .175\ci{.029}\sig & .787\ci{.115}\sig & .395\ci{.063}\sig & .292\ci{.031} & \second{.701}\ci{.024}\sig & .135\ci{.027}\sig & .803\ci{.098}\sig & .394\ci{.063}\sig \\
LIME\sa & .220\ci{.025}\sig & .719\ci{.027}\sig & .215\ci{.023}\sig & .746\ci{.090}\sig & .591\ci{.055}\sig & .275\ci{.028}\sig & .685\ci{.026}\sig & .168\ci{.024}\sig & .711\ci{.101}\sig & .558\ci{.062}\sig \\
KernelSHAP & .219\ci{.012}\sig & .674\ci{.016}\sig & .213\ci{.013}\sig & .802\ci{.040}\sig & \second{.670}\ci{.030}\sig & .329\ci{.015} & .652\ci{.015}\sig & .111\ci{.013}\sig & \best{.812}\ci{.044}\sig & \second{.682}\ci{.030}\sig \\
PartitionSHAP\sa & .173\ci{.021}\sig & .729\ci{.025}\sig & \second{.303}\ci{.026}\sig & \best{.895}\ci{.076}\sig & .537\ci{.059}\sig & .248\ci{.029}\sig & .697\ci{.024}\sig & \best{.225}\ci{.029}\sig & \second{.811}\ci{.091}\sig & .534\ci{.054}\sig \\
h-Shap & .355\ci{.011} & .586\ci{.017}\sig & .088\ci{.012}\sig & .731\ci{.049}\sig & \best{.724}\ci{.049}\sig & .451\ci{.013} & .576\ci{.017}\sig & .051\ci{.011}\sig & .698\ci{.052}\sig & \best{.692}\ci{.052}\sig \\
ShapBPT & \second{.171}\ci{.009}\sig & .713\ci{.014}\sig & .200\ci{.013}\sig & .778\ci{.044}\sig & .610\ci{.028}\sig & \best{.209}\ci{.010}\sig & .678\ci{.012}\sig & .084\ci{.014}\sig & .775\ci{.044}\sig & .593\ci{.027}\sig \\
Sobol\sa & .190\ci{.022}\sig & .678\ci{.031}\sig & .205\ci{.028}\sig & .721\ci{.115}\sig & .567\ci{.056}\sig & .290\ci{.029}\sig & .635\ci{.028}\sig & .095\ci{.030}\sig & .689\ci{.115}\sig & .513\ci{.055}\sig \\
HSIC & .226\ci{.012}\sig & .691\ci{.014}\sig & .232\ci{.016}\sig & .628\ci{.061}\sig & .531\ci{.028}\sig & .348\ci{.016} & .641\ci{.015}\sig & .117\ci{.015}\sig & .547\ci{.061}\sig & .506\ci{.030}\sig \\
LIMA\sa & .227\ci{.022}\sig & .695\ci{.028}\sig & .162\ci{.023}\sig & .629\ci{.109}\sig & .487\ci{.060}\sig & .332\ci{.028} & .654\ci{.028}\sig & .104\ci{.022}\sig & .669\ci{.106}\sig & .462\ci{.063}\sig \\
MoXI\sa & .295\ci{.028} & .677\ci{.030}\sig & .057\ci{.020}\sig & .407\ci{.120} & .377\ci{.065} & .354\ci{.031} & .639\ci{.030}\sig & .100\ci{.017}\sig & .463\ci{.126} & .384\ci{.067} \\
WCAM\sa & .292\ci{.027} & .670\ci{.030}\sig & .137\ci{.025}\sig & .607\ci{.131} & .476\ci{.054}\sig & .342\ci{.027} & .642\ci{.027}\sig & .059\ci{.024}\sig & .607\ci{.131} & .464\ci{.057}\sig \\
\addlinespace[2pt]
\tabgroup{11}{Ours}
\ours{\method} & \best{.151}\ci{.010}\sig & \second{.739}\ci{.012}\sig & \best{.343}\ci{.013}\sig & \second{.822}\ci{.053}\sig & .578\ci{.026}\sig & \second{.237}\ci{.014}\sig & \best{.706}\ci{.012}\sig & \second{.208}\ci{.015}\sig & .781\ci{.053}\sig & .546\ci{.026}\sig \\


==> tables/G503_realiad.tex <==
Occlusion & .801\ci{.041}\sig & .566\ci{.056}\sig & \second{.856}\ci{.028}\sig & .849\ci{.037}\sig & .380\ci{.058}\sig & .826\ci{.029}\sig & .847\ci{.030}\sig & .158\ci{.026}\sig & .823\ci{.024}\sig & .796\ci{.026}\sig & .086\ci{.016}\sig & .769\ci{.028}\sig \\
RISE\sa & \second{.935}\ci{.027}\sig & .091\ci{.017}\sig & .864\ci{.048}\sig & \best{.971}\ci{.014}\sig & .025\ci{.005}\sig & .803\ci{.049}\sig & \best{.968}\ci{.018}\sig & .007\ci{.001}\sig & \second{.788}\ci{.043}\sig & \best{.961}\ci{.020}\sig & .003\ci{.001}\sig & \second{.718}\ci{.050}\sig \\
LIME\sa & .731\ci{.030}\sig & .277\ci{.033}\sig & 1.087\ci{.067} & .684\ci{.031}\sig & .062\ci{.011}\sig & 1.146\ci{.085} & .692\ci{.032}\sig & .022\ci{.004}\sig & 1.162\ci{.066} & .692\ci{.044}\sig & .011\ci{.002}\sig & 1.125\ci{.084} \\
KernelSHAP & .880\ci{.024}\sig & .520\ci{.049}\sig & .873\ci{.032}\sig & .896\ci{.028}\sig & .306\ci{.047}\sig & .840\ci{.027}\sig & .814\ci{.036}\sig & .091\ci{.018}\sig & .870\ci{.030}\sig & .767\ci{.028}\sig & .053\ci{.011}\sig & .816\ci{.028}\sig \\
PartitionSHAP\sa & .859\ci{.027}\sig & \second{.771}\ci{.040}\sig & .868\ci{.080} & .889\ci{.036}\sig & \second{.719}\ci{.046}\sig & \best{.741}\ci{.046}\sig & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt \\
h-Shap & .515\ci{.012}\sig & .304\ci{.087}\sig & .918\ci{.024} & .571\ci{.024}\sig & .340\ci{.085}\sig & .905\ci{.031}\sig & .764\ci{.027}\sig & \second{.467}\ci{.063}\sig & .822\ci{.027}\sig & .805\ci{.026}\sig & \second{.316}\ci{.052}\sig & .759\ci{.031}\sig \\
ShapBPT & .899\ci{.026}\sig & .368\ci{.036}\sig & \na & .901\ci{.027}\sig & .179\ci{.029}\sig & \na & .859\ci{.036}\sig & .076\ci{.022}\sig & \na & \nrt & \nrt & \nrt \\
Sobol\sa & .894\ci{.024}\sig & .657\ci{.052}\sig & \na & .927\ci{.033}\sig & .487\ci{.050}\sig & \na & .940\ci{.025}\sig & .233\ci{.038}\sig & \na & .906\ci{.023}\sig & .127\ci{.022}\sig & \na \\
HSIC & .904\ci{.024}\sig & .552\ci{.055}\sig & \na & .946\ci{.019}\sig & .316\ci{.047}\sig & \na & .892\ci{.029}\sig & .112\ci{.018}\sig & \na & .838\ci{.026}\sig & .058\ci{.011}\sig & \na \\
LIMA\sa & .756\ci{.046}\sig & .106\ci{.025}\sig & .891\ci{.023}\sig & .788\ci{.046}\sig & .029\ci{.006}\sig & .881\ci{.026}\sig & .738\ci{.048}\sig & .007\ci{.002}\sig & .907\ci{.021}\sig & .673\ci{.065}\sig & .003\ci{.001}\sig & .880\ci{.031} \\
MoXI\sa & .661\ci{.043}\sig & .093\ci{.016}\sig & .941\ci{.035} & .768\ci{.042}\sig & .026\ci{.004}\sig & .883\ci{.045}\sig & .826\ci{.042}\sig & .008\ci{.001}\sig & .899\ci{.045}\sig & .806\ci{.040}\sig & .004\ci{.001}\sig & .861\ci{.037} \\
WCAM\sa & .863\ci{.036}\sig & .261\ci{.041}\sig & .893\ci{.024}\sig & .831\ci{.036}\sig & .094\ci{.018}\sig & .880\ci{.027}\sig & .720\ci{.040}\sig & .023\ci{.005}\sig & .896\ci{.023}\sig & .674\ci{.029}\sig & .011\ci{.003}\sig & .837\ci{.019}\sig \\
\ours{\method} & \best{.944}\ci{.022}\sig & \best{.910}\ci{.046}\sig & \best{.819}\ci{.036}\sig & \second{.962}\ci{.024}\sig & \best{.900}\ci{.048}\sig & \second{.761}\ci{.043}\sig & \second{.963}\ci{.024}\sig & \best{.872}\ci{.055}\sig & \best{.714}\ci{.038}\sig & \second{.959}\ci{.022}\sig & \best{.898}\ci{.049}\sig & \best{.656}\ci{.046}\sig \\


==> tables/G503_visa_a.tex <==
Occlusion & .745\ci{.046}\sig & .359\ci{.066}\sig & \best{.812}\ci{.063} & .771\ci{.185} & .250\ci{.217} & 1.558\ci{.753} & .714\ci{.059}\sig & .270\ci{.126}\sig & .793\ci{.050}\sig & .792\ci{.055}\sig & .246\ci{.069}\sig & .761\ci{.112} \\
RISE\sa & \best{.915}\ci{.029}\sig & .047\ci{.013}\sig & .901\ci{.110} & \best{.903}\ci{.086} & .014\ci{.010} & \second{.680}\ci{.200} & \best{.888}\ci{.044}\sig & .045\ci{.044}\sig & \second{.768}\ci{.078} & \second{.928}\ci{.039}\sig & .014\ci{.005}\sig & .920\ci{.238} \\
LIME\sa & .650\ci{.060}\sig & .162\ci{.033}\sig & .942\ci{.091} & .716\ci{.184} & .051\ci{.044} & 1.019\ci{.398} & .713\ci{.072}\sig & .063\ci{.049}\sig & 1.016\ci{.097} & .641\ci{.060}\sig & .037\ci{.010}\sig & .841\ci{.320} \\
KernelSHAP & .673\ci{.042}\sig & .154\ci{.049}\sig & .858\ci{.101} & .790\ci{.119} & .327\ci{.262} & 1.701\ci{.986} & .675\ci{.069}\sig & .112\ci{.098}\sig & .923\ci{.047} & .694\ci{.056}\sig & .074\ci{.048}\sig & .874\ci{.107} \\
PartitionSHAP\sa & .849\ci{.034}\sig & .389\ci{.059}\sig & .842\ci{.078} & .756\ci{.178} & \best{.480}\ci{.258} & .800\ci{.396} & .807\ci{.065}\sig & .258\ci{.116}\sig & .894\ci{.095} & .887\ci{.039}\sig & .382\ci{.069}\sig & \best{.638}\ci{.302}\sig \\
h-Shap & .601\ci{.027}\sig & \second{.558}\ci{.081}\sig & .877\ci{.087} & .566\ci{.056} & .279\ci{.250} & 1.630\ci{.809} & .688\ci{.052}\sig & \second{.402}\ci{.112}\sig & .816\ci{.061} & .646\ci{.036}\sig & \second{.442}\ci{.104}\sig & \second{.711}\ci{.292}\sig \\
ShapBPT & .898\ci{.029}\sig & .256\ci{.049}\sig & \na & .818\ci{.207} & .241\ci{.209} & \na & .874\ci{.052}\sig & .184\ci{.098}\sig & \na & .886\ci{.041}\sig & .148\ci{.047}\sig & \na \\
Sobol\sa & .878\ci{.031}\sig & .417\ci{.066}\sig & \na & \second{.877}\ci{.135} & .201\ci{.156} & \na & .874\ci{.044}\sig & .277\ci{.104}\sig & \na & .875\ci{.053}\sig & .284\ci{.079}\sig & \na \\
HSIC & .865\ci{.031}\sig & .322\ci{.059}\sig & \na & .859\ci{.165} & .173\ci{.143} & \na & .806\ci{.054}\sig & .216\ci{.108}\sig & \na & .901\ci{.039}\sig & .192\ci{.058}\sig & \na \\
LIMA\sa & .786\ci{.039}\sig & .081\ci{.025}\sig & .840\ci{.083} & .754\ci{.176} & .030\ci{.027} & 1.097\ci{.364} & .723\ci{.065}\sig & .061\ci{.046}\sig & .815\ci{.065} & .814\ci{.057}\sig & .027\ci{.011}\sig & .759\ci{.255} \\
MoXI\sa & .576\ci{.051}\sig & .041\ci{.012} & 1.010\ci{.063} & .683\ci{.122} & .014\ci{.009} & .982\ci{.170} & .654\ci{.095}\sig & .041\ci{.040} & .921\ci{.064} & .760\ci{.059}\sig & .015\ci{.006}\sig & .967\ci{.139} \\
WCAM\sa & .833\ci{.032}\sig & .151\ci{.040}\sig & .887\ci{.040} & .824\ci{.131} & .066\ci{.053} & .875\ci{.177} & .799\ci{.046}\sig & .106\ci{.078}\sig & .813\ci{.065} & .812\ci{.048}\sig & .066\ci{.025}\sig & .891\ci{.092} \\
\ours{\method} & \second{.900}\ci{.029}\sig & \best{.678}\ci{.082}\sig & \second{.828}\ci{.082} & .856\ci{.169} & \second{.456}\ci{.320} & \best{.595}\ci{.146} & \second{.886}\ci{.050}\sig & \best{.674}\ci{.114}\sig & \best{.729}\ci{.065}\sig & \best{.941}\ci{.034}\sig & \best{.683}\ci{.107}\sig & .815\ci{.144} \\


==> tables/G503_visa_b.tex <==
Occlusion & .869\ci{.054}\sig & .228\ci{.079}\sig & .397\ci{.206} & .883\ci{.045}\sig & .338\ci{.173}\sig & \best{.843}\ci{.056}\sig & .568\ci{.186} & .058\ci{.029} & \best{.730}\ci{.083} & .807\ci{.071}\sig & .150\ci{.074}\sig & .916\ci{.161}\sig \\
RISE\sa & .931\ci{.062}\sig & .012\ci{.008}\sig & .514\ci{.131} & \best{.984}\ci{.006}\sig & .018\ci{.012}\sig & .934\ci{.058} & \best{.954}\ci{.058} & .008\ci{.006} & 1.604\ci{1.318} & \second{.880}\ci{.078}\sig & .008\ci{.005}\sig & \second{.853}\ci{.122} \\
LIME\sa & .800\ci{.088}\sig & .044\ci{.015}\sig & .414\ci{.245} & .483\ci{.123} & .035\ci{.019}\sig & 1.046\ci{.060} & .663\ci{.175} & .034\ci{.023} & 1.055\ci{.530} & .579\ci{.063} & .021\ci{.012}\sig & .995\ci{.123} \\
KernelSHAP & .814\ci{.120}\sig & .174\ci{.117}\sig & .433\ci{.179} & .597\ci{.115} & .045\ci{.042}\sig & .965\ci{.026} & .591\ci{.103} & .012\ci{.014} & .916\ci{.065} & .693\ci{.103}\sig & .032\ci{.023}\sig & .957\ci{.085} \\
PartitionSHAP\sa & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt & \nrt \\
h-Shap & .683\ci{.060}\sig & \second{.549}\ci{.179}\sig & \second{.345}\ci{.239}\sig & .634\ci{.059}\sig & \second{.551}\ci{.203}\sig & \second{.897}\ci{.058}\sig & .745\ci{.123} & \second{.356}\ci{.166} & \second{.737}\ci{.233} & .656\ci{.072}\sig & \second{.299}\ci{.135}\sig & .912\ci{.199}\sig \\
ShapBPT & .879\ci{.089}\sig & .184\ci{.094}\sig & \na & .907\ci{.051}\sig & .166\ci{.088}\sig & \na & .942\ci{.059} & .174\ci{.077} & \na & .807\ci{.088}\sig & .051\ci{.027}\sig & \na \\
Sobol\sa & \best{.944}\ci{.046}\sig & .311\ci{.109}\sig & \na & .931\ci{.040}\sig & .352\ci{.163}\sig & \na & .878\ci{.116} & .154\ci{.084} & \na & .834\ci{.129}\sig & .173\ci{.092}\sig & \na \\
HSIC & .916\ci{.053}\sig & .169\ci{.065}\sig & \na & .942\ci{.045}\sig & .262\ci{.136}\sig & \na & .839\ci{.134} & .064\ci{.026} & \na & .786\ci{.107}\sig & .102\ci{.058}\sig & \na \\
LIMA\sa & .869\ci{.040}\sig & .034\ci{.020}\sig & .453\ci{.148} & .850\ci{.076}\sig & .026\ci{.021}\sig & .921\ci{.057} & .810\ci{.127} & .040\ci{.057} & .852\ci{.351} & .763\ci{.088}\sig & .016\ci{.009}\sig & .916\ci{.190}\sig \\
MoXI\sa & .678\ci{.123}\sig & .011\ci{.007} & .587\ci{.252} & .883\ci{.069}\sig & .022\ci{.013}\sig & .904\ci{.048} & .669\ci{.152} & .007\ci{.005} & 1.343\ci{.900} & .512\ci{.117} & .005\ci{.003} & .969\ci{.110} \\
WCAM\sa & .890\ci{.039}\sig & .067\ci{.044}\sig & .672\ci{.065} & .880\ci{.068}\sig & .088\ci{.060}\sig & .963\ci{.049} & .824\ci{.083} & .033\ci{.020} & 1.086\ci{.414} & .703\ci{.097}\sig & .031\ci{.021}\sig & .879\ci{.070} \\
\ours{\method} & \second{.938}\ci{.058}\sig & \best{.668}\ci{.214}\sig & \best{.327}\ci{.200}\sig & \second{.966}\ci{.023}\sig & \best{.712}\ci{.226}\sig & .902\ci{.051} & \second{.944}\ci{.055} & \best{.752}\ci{.250} & 1.106\ci{.672} & \best{.918}\ci{.078}\sig & \best{.564}\ci{.203}\sig & \best{.830}\ci{.152} \\


==> tables/G507_gridpg_2up.tex <==
\multicolumn{4}{@{}l}{\tabheadfont Perturbation-based} & & \multicolumn{4}{@{}l}{\tabheadfont References} \\
Occlusion & .617\ci{.009}\sig & .695\ci{.007}\sig & .655\ci{.005} & & \ctrl{Random map} & \ctrl{.250\ci{.000}} & \ctrl{.250\ci{.000}} & \ctrl{.250\ci{.000}} \\
RISE\sa & .277\ci{.001}\sig & .284\ci{.001}\sig & .280\ci{.001} & & \ctrl{Centre map} & \ctrl{.250\ci{.000}} & \ctrl{.250\ci{.000}} & \ctrl{.250\ci{.000}} \\
LIME\sa & .662\ci{.010}\sig & .592\ci{.012}\sig & .627\ci{.009} & & \multicolumn{4}{@{}l}{\tabheadfont Gradient- and activation-based} \\
KernelSHAP & \second{.872}\ci{.005}\sig & .817\ci{.010}\sig & \second{.846}\ci{.006} & & Saliency & .451\ci{.004}\sig & .434\ci{.005}\sig & \na \\
PartitionSHAP\sa & .694\ci{.016}\sig & .802\ci{.014}\sig & .748\ci{.011} & & Integrated Gradients & .429\ci{.006}\sig & .395\ci{.005}\sig & \na \\
h-Shap & .831\ci{.017}\sig & .760\ci{.020}\sig & .797\ci{.013} & & SmoothGrad & .548\ci{.007}\sig & .417\ci{.007}\sig & \na \\
ShapBPT & .860\ci{.005}\sig & \second{.825}\ci{.006}\sig & .844\ci{.004} & & Grad-CAM & .816\ci{.005}\sig & .769\ci{.006}\sig & \na \\
Sobol\sa & .705\ci{.016}\sig & .667\ci{.018}\sig & .686\ci{.012} & & Grad-CAM++ & .427\ci{.002}\sig & .392\ci{.004}\sig & \na \\
HSIC & .826\ci{.006}\sig & .744\ci{.009}\sig & .787\ci{.005} & & & & & \\
LIMA\sa & .388\ci{.006}\sig & .384\ci{.005}\sig & .386\ci{.004} & & & & & \\
MoXI\sa & .292\ci{.005}\sig & .325\ci{.003}\sig & .309\ci{.003} & & & & & \\
WCAM\sa & .613\ci{.018}\sig & .527\ci{.017}\sig & .570\ci{.012} & & & & & \\
\multicolumn{4}{@{}l}{\tabheadfont Ours} & & & & & \\
\ours{\method} & \best{.915}\ci{.008}\sig & \best{.896}\ci{.008}\sig & \best{.905}\ci{.006} & & & & & \\


==> tables/G507_synth_t.tex <==
\multicolumn{14}{@{}l}{\tabheadfont attention pooling, $s=32$\,px}\\[1pt]
256 & .967\ci{.005}\sig & \best{.999}\ci{.000}\sig & .882\ci{.046}\sig & .931\ci{.011}\sig & .846\ci{.037}\sig & .672\ci{.018}\sig & .975\ci{.004}\sig & .995\ci{.003}\sig & .988\ci{.002}\sig & .910\ci{.019}\sig & .896\ci{.043} & .990\ci{.006} & \second{.998}\ci{.000}\sig \\
512 & .953\ci{.005}\sig & \best{.999}\ci{.000}\sig & .912\ci{.032}\sig & .937\ci{.009}\sig & .887\ci{.029}\sig & .825\ci{.019}\sig & .965\ci{.004}\sig & .990\ci{.003}\sig & .972\ci{.004}\sig & .893\ci{.038}\sig & .893\ci{.074} & .994\ci{.004} & \second{.996}\ci{.000}\sig \\
1024 & .835\ci{.011}\sig & \best{.993}\ci{.002}\sig & .925\ci{.023}\sig & .832\ci{.015}\sig & .919\ci{.030}\sig & .899\ci{.019}\sig & .916\ci{.008}\sig & .957\ci{.010}\sig & .852\ci{.015}\sig & .831\ci{.028}\sig & .838\ci{.201} & .922\ci{.031} & \second{.991}\ci{.002}\sig \\
2048 & .652\ci{.021}\sig & \best{.987}\ci{.007}\sig & .901\ci{.090}\sig & .684\ci{.025}\sig & \nrt & .871\ci{.027}\sig & .829\ci{.020}\sig & .797\ci{.070}\sig & .796\ci{.035}\sig & .681\ci{.055}\sig & .774\ci{.169} & .961\ci{.035} & \second{.987}\ci{.004}\sig \\
4096 & .500\ci{.000} & \best{.985}\ci{.008}\sig & .953\ci{.037} & .568\ci{.033}\sig & \nrt & .742\ci{.020}\sig & \nrt & .795\ci{.070}\sig & .796\ci{.035}\sig & .622\ci{.084} & .554\ci{.048} & .916\ci{.045} & \second{.984}\ci{.006}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE pooling, $s=32$\,px}\\[1pt]
256 & .963\ci{.006}\sig & \best{.999}\ci{.000}\sig & .925\ci{.024}\sig & .962\ci{.006}\sig & .900\ci{.024}\sig & .624\ci{.001}\sig & .978\ci{.002}\sig & .996\ci{.001}\sig & .989\ci{.001}\sig & .921\ci{.041}\sig & .927\ci{.041} & .993\ci{.004} & \second{.997}\ci{.000}\sig \\
512 & .953\ci{.007}\sig & \best{.999}\ci{.000}\sig & .948\ci{.020}\sig & .947\ci{.007}\sig & .914\ci{.026}\sig & .773\ci{.015}\sig & .971\ci{.004}\sig & .990\ci{.003}\sig & .977\ci{.003}\sig & .941\ci{.017}\sig & .928\ci{.035} & .987\ci{.017} & \second{.996}\ci{.000}\sig \\
1024 & .823\ci{.014}\sig & \best{.994}\ci{.002}\sig & .918\ci{.035}\sig & .819\ci{.016}\sig & .927\ci{.034}\sig & .867\ci{.023}\sig & .915\ci{.008}\sig & .958\ci{.012}\sig & .850\ci{.015}\sig & .830\ci{.029}\sig & .869\ci{.058} & .937\ci{.040} & \second{.991}\ci{.001}\sig \\
2048 & .648\ci{.019}\sig & \best{.987}\ci{.004}\sig & .947\ci{.018}\sig & .678\ci{.036}\sig & \nrt & .850\ci{.029}\sig & .803\ci{.031}\sig & .842\ci{.058}\sig & .798\ci{.037}\sig & .691\ci{.045}\sig & .720\ci{.092} & .932\ci{.053} & \second{.984}\ci{.006}\sig \\
4096 & .500\ci{.000} & \best{.980}\ci{.010}\sig & .944\ci{.039} & .573\ci{.027}\sig & \nrt & .728\ci{.026}\sig & \nrt & .823\ci{.064}\sig & .797\ci{.037}\sig & .527\ci{.044} & .519\ci{.058} & .867\ci{.054} & \second{.978}\ci{.011}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont max pooling, $s=32$\,px}\\[1pt]
256 & .965\ci{.004}\sig & \best{.999}\ci{.000}\sig & .923\ci{.017}\sig & .965\ci{.003}\sig & .887\ci{.027}\sig & .620\ci{.003}\sig & .977\ci{.001}\sig & .996\ci{.001}\sig & .988\ci{.001}\sig & .895\ci{.025}\sig & .817\ci{.192} & .994\ci{.003} & \second{.997}\ci{.000}\sig \\
512 & .958\ci{.003}\sig & \best{.999}\ci{.000}\sig & .934\ci{.017}\sig & .944\ci{.004}\sig & .911\ci{.025}\sig & .776\ci{.010}\sig & .968\ci{.002}\sig & .990\ci{.002}\sig & .974\ci{.002}\sig & .948\ci{.014}\sig & .983\ci{.019} & \second{.998}\ci{.001} & .996\ci{.000}\sig \\
1024 & .823\ci{.009}\sig & \best{.994}\ci{.001}\sig & .923\ci{.022}\sig & .820\ci{.009}\sig & .926\ci{.024}\sig & .866\ci{.014}\sig & .913\ci{.005}\sig & .958\ci{.006}\sig & .838\ci{.009}\sig & .842\ci{.019}\sig & .961\ci{.030} & .930\ci{.053} & \second{.991}\ci{.001}\sig \\
2048 & .656\ci{.027}\sig & \best{.982}\ci{.008}\sig & .907\ci{.074}\sig & .681\ci{.050}\sig & \nrt & .822\ci{.045}\sig & .825\ci{.022}\sig & .793\ci{.098}\sig & .781\ci{.045}\sig & .715\ci{.039}\sig & .928\ci{.039} & .868\ci{.098} & \second{.977}\ci{.008}\sig \\
4096 & .500\ci{.000} & \second{.962}\ci{.026}\sig & .895\ci{.099} & .570\ci{.029}\sig & \nrt & .695\ci{.028}\sig & \nrt & .788\ci{.099}\sig & .781\ci{.045}\sig & .558\ci{.079} & .564\ci{.067} & .913\ci{.077} & \best{.966}\ci{.014}\sig \\
8192 & .549\ci{.021}\sig & .709\ci{.051}\sig & \second{.871}\ci{.103} & .561\ci{.030}\sig & \nrt & .616\ci{.038}\sig & \nrt & .554\ci{.018}\sig & .531\ci{.005}\sig & \nrt & .530\ci{.030} & .622\ci{.069} & \best{.978}\ci{.010}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE, large receptive field, $s=32$\,px}\\[1pt]
256 & .956\ci{.009}\sig & \best{.999}\ci{.000}\sig & .911\ci{.026}\sig & .962\ci{.006}\sig & .890\ci{.030}\sig & .634\ci{.013}\sig & .976\ci{.002}\sig & .996\ci{.001}\sig & .988\ci{.002}\sig & .903\ci{.035}\sig & .951\ci{.024} & .989\ci{.011} & \second{.997}\ci{.000}\sig \\
512 & .955\ci{.005}\sig & \best{.999}\ci{.000}\sig & .936\ci{.023}\sig & .935\ci{.009}\sig & .921\ci{.024}\sig & .784\ci{.015}\sig & .966\ci{.004}\sig & .992\ci{.002}\sig & .977\ci{.003}\sig & .907\ci{.042}\sig & .914\ci{.097} & .989\ci{.011} & \second{.997}\ci{.000}\sig \\
1024 & .825\ci{.015}\sig & \best{.993}\ci{.001}\sig & .916\ci{.033}\sig & .815\ci{.016}\sig & .922\ci{.025}\sig & .873\ci{.020}\sig & .911\ci{.008}\sig & .950\ci{.013}\sig & .854\ci{.015}\sig & .806\ci{.024}\sig & .832\ci{.147} & .911\ci{.023} & \second{.991}\ci{.001}\sig \\
2048 & .656\ci{.018}\sig & \second{.978}\ci{.008}\sig & .956\ci{.033}\sig & .674\ci{.048}\sig & \nrt & .870\ci{.028}\sig & .811\ci{.022}\sig & .784\ci{.056}\sig & .788\ci{.034}\sig & .680\ci{.038}\sig & .775\ci{.104} & .901\ci{.052} & \best{.983}\ci{.006}\sig \\
4096 & .500\ci{.000} & .952\ci{.025}\sig & \second{.973}\ci{.009} & .598\ci{.034}\sig & \nrt & .741\ci{.025}\sig & \nrt & .785\ci{.055}\sig & .788\ci{.034}\sig & .561\ci{.053} & .538\ci{.113} & .941\ci{.050} & \best{.976}\ci{.012}\sig \\
8192 & .572\ci{.059} & .702\ci{.054}\sig & \second{.910}\ci{.121} & .569\ci{.037}\sig & \nrt & .590\ci{.056} & \nrt & .570\ci{.026}\sig & .589\ci{.080}\sig & \nrt & .525\ci{.103} & .663\ci{.192} & \best{.989}\ci{.009}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE, large receptive field, fine-tuned, $s=16$\,px}\\[1pt]
512 & .833\ci{.013}\sig & \best{.995}\ci{.001}\sig & .903\ci{.022}\sig & .781\ci{.023}\sig & .945\ci{.023}\sig & .886\ci{.017}\sig & .913\ci{.009}\sig & .952\ci{.012}\sig & .855\ci{.017}\sig & .759\ci{.061}\sig & .857\ci{.054} & .974\ci{.009} & \second{.990}\ci{.002}\sig \\
1024 & .701\ci{.015}\sig & \best{.981}\ci{.006}\sig & .892\ci{.028}\sig & .670\ci{.020}\sig & .946\ci{.018}\sig & .855\ci{.016}\sig & .812\ci{.014}\sig & .868\ci{.038}\sig & .715\ci{.019}\sig & .663\ci{.039}\sig & .741\ci{.200} & .797\ci{.090} & \second{.981}\ci{.005}\sig \\
2048 & .637\ci{.030}\sig & .894\ci{.051}\sig & \second{.895}\ci{.075}\sig & .579\ci{.051}\sig & \nrt & .712\ci{.017}\sig & .685\ci{.031}\sig & .695\ci{.093}\sig & .579\ci{.008}\sig & .535\ci{.056} & .784\ci{.140} & .730\ci{.131} & \best{.980}\ci{.010}\sig \\
4096 & .500\ci{.000} & .834\ci{.077}\sig & \second{.929}\ci{.012} & .534\ci{.028}\sig & \nrt & .573\ci{.024}\sig & \nrt & .579\ci{.014}\sig & .562\ci{.008}\sig & .480\ci{.054} & .523\ci{.200} & .626\ci{.034} & \best{.977}\ci{.013}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE, large receptive field, fine-tuned, $s=64$\,px}\\[1pt]
512 & .975\ci{.003}\sig & \best{.999}\ci{.000}\sig & .965\ci{.008}\sig & .940\ci{.009}\sig & .916\ci{.037}\sig & .648\ci{.011}\sig & .976\ci{.002}\sig & .996\ci{.002}\sig & .990\ci{.001}\sig & .926\ci{.026}\sig & .954\ci{.034} & \second{.997}\ci{.001} & .997\ci{.000}\sig \\
1024 & .955\ci{.004}\sig & \best{.999}\ci{.000}\sig & .949\ci{.013}\sig & .929\ci{.007}\sig & .912\ci{.034}\sig & .795\ci{.015}\sig & .964\ci{.003}\sig & .990\ci{.002}\sig & .974\ci{.003}\sig & .946\ci{.013}\sig & \second{.998}\ci{.001} & .979\ci{.015} & .996\ci{.000}\sig \\
2048 & .816\ci{.029}\sig & \best{.995}\ci{.002}\sig & .966\ci{.009}\sig & .811\ci{.026}\sig & \nrt & .862\ci{.032}\sig & .897\ci{.017}\sig & .955\ci{.010}\sig & .870\ci{.027}\sig & .818\ci{.053}\sig & .947\ci{.025} & .848\ci{.078} & \second{.994}\ci{.001}\sig \\
4096 & .657\ci{.022}\sig & \second{.987}\ci{.008}\sig & .972\ci{.012} & .678\ci{.041}\sig & \nrt & .855\ci{.029}\sig & \nrt & .823\ci{.082}\sig & .783\ci{.039}\sig & .658\ci{.003} & .837\ci{.139} & .869\ci{.085} & \best{.992}\ci{.004}\sig \\
8192 & .618\ci{.070} & \second{.934}\ci{.038}\sig & .876\ci{.088} & .594\ci{.089} & \nrt & .672\ci{.061}\sig & \nrt & .700\ci{.085}\sig & .596\ci{.021}\sig & \nrt & .506\ci{.104} & .634\ci{.121} & \best{.978}\ci{.027}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE, large receptive field, fine-tuned, $s=128$\,px}\\[1pt]
1024 & .976\ci{.002}\sig & \best{.999}\ci{.000}\sig & .840\ci{.032}\sig & .945\ci{.009}\sig & .925\ci{.032}\sig & .656\ci{.010}\sig & .972\ci{.003}\sig & \second{.996}\ci{.001}\sig & .988\ci{.002}\sig & .922\ci{.021}\sig & .936\ci{.109} & .942\ci{.074} & .996\ci{.000}\sig \\
2048 & .963\ci{.004}\sig & \best{.999}\ci{.000}\sig & .870\ci{.029}\sig & .920\ci{.015}\sig & \nrt & .768\ci{.039}\sig & .962\ci{.006}\sig & .990\ci{.005}\sig & .977\ci{.004}\sig & .940\ci{.024}\sig & .984\ci{.009} & .751\ci{.253} & \second{.997}\ci{.001}\sig \\
4096 & .829\ci{.016}\sig & \best{.995}\ci{.002}\sig & .871\ci{.028} & .821\ci{.021}\sig & \nrt & .867\ci{.045}\sig & \nrt & .967\ci{.011}\sig & .829\ci{.025}\sig & .873\ci{.023} & .893\ci{.038} & .628\ci{.211} & \second{.995}\ci{.002}\sig \\
\midrule
\multicolumn{14}{@{}l}{\tabheadfont LSE, large receptive field, fine-tuned, $s=256$\,px}\\[1pt]
2048 & .960\ci{.012}\sig & \best{.999}\ci{.001}\sig & .675\ci{.014}\sig & .917\ci{.023}\sig & \nrt & .623\ci{.002}\sig & .965\ci{.005}\sig & \second{.997}\ci{.002}\sig & .990\ci{.003}\sig & .931\ci{.034}\sig & .956\ci{.024} & .986\ci{.011} & .996\ci{.001}\sig \\
4096 & .954\ci{.009}\sig & \best{.998}\ci{.001}\sig & .680\ci{.036} & .929\ci{.015}\sig & \nrt & .780\ci{.029}\sig & \nrt & .991\ci{.004}\sig & .975\ci{.006}\sig & .946\ci{.020} & .973\ci{.015} & .970\ci{.014} & \second{.996}\ci{.001}\sig \\


==> tables/S_same_sides.tex <==
Occlusion & 252 & $+.383$\dci{$+.341$}{$+.428$} & $+.497$\dci{$+.451$}{$+.552$} & 368 & $+.597$\dci{$+.567$}{$+.628$} & $+.619$\dci{$+.580$}{$+.657$} & 384 & $+.096$\dci{$+.073$}{$+.122$} & $+.306$\dci{$+.262$}{$+.351$} \\
RISE & 255 & $+.638$\dci{$+.590$}{$+.685$} & $+.208$\dci{$+.140$}{$+.274$} & 368 & $+.864$\dci{$+.840$}{$+.886$} & $+.154$\dci{$+.106$}{$+.203$} & 331 & $+.175$\dci{$+.139$}{$+.212$} & $+.198$\dci{$+.133$}{$+.267$} \\
LIME & 251 & $+.577$\dci{$+.532$}{$+.621$} & $+.327$\dci{$+.273$}{$+.381$} & 328 & $+.790$\dci{$+.762$}{$+.817$} & $+.278$\dci{$+.233$}{$+.327$} & 292 & $+.159$\dci{$+.120$}{$+.201$} & $+.234$\dci{$+.175$}{$+.287$} \\
KernelSHAP & 241 & $+.574$\dci{$+.526$}{$+.622$} & $+.561$\dci{$+.510$}{$+.613$} & 368 & $+.652$\dci{$+.623$}{$+.682$} & $+.612$\dci{$+.573$}{$+.649$} & 380 & $+.060$\dci{$+.033$}{$+.089$} & $+.223$\dci{$+.173$}{$+.273$} \\
PartitionSHAP & 197 & $+.302$\dci{$+.256$}{$+.345$} & $+.184$\dci{$+.125$}{$+.243$} & 184 & $+.160$\dci{$+.135$}{$+.186$} & $+.073$\dci{$+.017$}{$+.133$} & 168 & $+.035$\nsd\dci{$-.003$}{$+.074$} & $+.050$\nsd\dci{$-.026$}{$+.121$} \\
h-Shap & 255 & $+.191$\dci{$+.154$}{$+.229$} & $+.315$\dci{$+.265$}{$+.369$} & 348 & $+.538$\dci{$+.500$}{$+.575$} & $+.610$\dci{$+.567$}{$+.651$} & 370 & $+.038$\dci{$+.011$}{$+.066$} & $+.199$\dci{$+.154$}{$+.246$} \\
ShapBPT & 255 & $+.473$\dci{$+.429$}{$+.517$} & $+.354$\dci{$+.297$}{$+.409$} & 276 & $+.686$\dci{$+.655$}{$+.717$} & $+.506$\dci{$+.449$}{$+.560$} & 264 & $+.076$\dci{$+.045$}{$+.112$} & $+.157$\dci{$+.099$}{$+.213$} \\
Sobol & 255 & $+.342$\dci{$+.303$}{$+.384$} & $+.310$\dci{$+.239$}{$+.381$} & 368 & $+.519$\dci{$+.490$}{$+.549$} & $+.349$\dci{$+.291$}{$+.405$} & 383 & $+.054$\dci{$+.031$}{$+.078$} & $+.055$\nsd\dci{$+.002$}{$+.114$} \\
HSIC & 255 & $+.431$\dci{$+.386$}{$+.474$} & $+.397$\dci{$+.332$}{$+.464$} & 368 & $+.635$\dci{$+.606$}{$+.666$} & $+.505$\dci{$+.456$}{$+.556$} & 384 & $+.093$\dci{$+.067$}{$+.120$} & $+.193$\dci{$+.135$}{$+.256$} \\
LIMA & 255 & $+.615$\dci{$+.568$}{$+.662$} & $+.522$\dci{$+.472$}{$+.573$} & 296 & $+.848$\dci{$+.820$}{$+.876$} & $+.743$\dci{$+.698$}{$+.788$} & 258 & $+.133$\dci{$+.099$}{$+.176$} & $+.285$\dci{$+.225$}{$+.346$} \\
MoXI & 255 & $+.640$\dci{$+.592$}{$+.688$} & $+.400$\dci{$+.339$}{$+.462$} & 368 & $+.862$\dci{$+.838$}{$+.885$} & $+.500$\dci{$+.448$}{$+.555$} & 294 & $+.189$\dci{$+.148$}{$+.231$} & $+.127$\dci{$+.061$}{$+.202$} \\
WCAM & 255 & $+.566$\dci{$+.522$}{$+.612$} & $+.514$\dci{$+.448$}{$+.578$} & 368 & $+.798$\dci{$+.772$}{$+.822$} & $+.715$\dci{$+.669$}{$+.759$} & 314 & $+.148$\dci{$+.115$}{$+.186$} & $+.137$\dci{$+.074$}{$+.207$} \\


==> tables/T2_hr_body.tex <==
\ctrl{Random map} & \ctrl{.500\ci{.001}} & \ctrl{.019\ci{.006}} & \ctrl{.956\ci{.138}} & \ctrl{.500\ci{.000}} & \ctrl{.029\ci{.005}} & \ctrl{.927\ci{.011}} & \ctrl{.500\ci{.001}} & \ctrl{.047\ci{.010}} & \ctrl{.899\ci{.014}} & \ctrl{.509\ci{.035}} & \ctrl{0} &  \\
\ctrl{Centre map} & \ctrl{.688\ci{.023}} & \ctrl{.034\ci{.010}} & \ctrl{.986\ci{.121}} & \ctrl{.671\ci{.017}} & \ctrl{.047\ci{.008}} & \ctrl{.922\ci{.011}} & \ctrl{.681\ci{.015}} & \ctrl{.083\ci{.016}} & \ctrl{.946\ci{.014}} & \ctrl{.564\ci{.045}} & \ctrl{0} &  \\
\midrule
Occlusion & .769\ci{.035} & .237\ci{.043} & .851\ci{.108}\nsd & .823\ci{.017} & .298\ci{.021} & .818\ci{.014} & .568\ci{.026} & .120\ci{.026} & .848\ci{.024} & .625\ci{.057} & \best{0.6} & $L^2$ \\
RISE & \best{.923}\ci{.018}\nsd & .021\ci{.006} & .897\ci{.173} & \best{.959}\ci{.010}\nsd & .031\ci{.005} & \second{.793}\ci{.022} & .620\ci{.030} & .049\ci{.010} & .860\ci{.016} & .608\ci{.047} & 38,691 & none \\
LIME & .656\ci{.042} & .056\ci{.010} & .916\ci{.098} & .700\ci{.016} & .093\ci{.009} & 1.130\ci{.037} & .599\ci{.019} & .064\ci{.013} & .871\ci{.030} & .744\ci{.062} & 6,390 & none \\
KernelSHAP & .691\ci{.033} & .116\ci{.038} & .953\ci{.120} & .839\ci{.016} & .243\ci{.017} & .850\ci{.015} & .662\ci{.025}\nsd & .148\ci{.023} & .837\ci{.015} & .778\ci{.051} & 80.1 & $L^2$ \\
PartitionSHAP & .825\ci{.051} & .377\ci{.073} & .794\ci{.124}\nsd & .874\ci{.021} & \second{.745}\ci{.030} & .804\ci{.047}\nsd & .697\ci{.028}\nsd & \best{.244}\ci{.042}\nsd & \best{.750}\ci{.035}\nsd & .736\ci{.035} & \second{2.4} & $k\log L$ \\
h-Shap & .652\ci{.024} & \second{.429}\ci{.055} & .866\ci{.115}\nsd & .664\ci{.011} & .357\ci{.038} & .851\ci{.014} & .560\ci{.027} & .185\ci{.056} & .852\ci{.019} & \second{.922}\ci{.013}\nsd & 255 & $k\log L$ \\
ShapBPT & .876\ci{.029} & .176\ci{.035} & .870\ci{.111}\nsd & .886\ci{.019} & .208\ci{.017} & \na & \second{.739}\ci{.025} & .178\ci{.028} & .802\ci{.027} & \na & \na & $k\log L$ \\
Sobol & .886\ci{.027} & .271\ci{.041} & \best{.736}\ci{.064}\nsd & .917\ci{.013} & .376\ci{.021} & \na & \best{.752}\ci{.024} & .157\ci{.029} & .896\ci{.052}\nsd & \na & 16,361 & $L^2$ \\
HSIC & .864\ci{.028} & .187\ci{.032} & .875\ci{.080} & .895\ci{.013} & .260\ci{.019} & \na & .683\ci{.022}\nsd & .120\ci{.022} & .907\ci{.024} & .797\ci{.043} & 766 & none \\
LIMA & .796\ci{.036} & .039\ci{.011} & .832\ci{.076}\nsd & .739\ci{.026} & .036\ci{.006} & .890\ci{.012} & .629\ci{.029} & .096\ci{.025} & .827\ci{.022} & .725\ci{.055} & 982 & $L^4$ \\
MoXI & .677\ci{.036} & .019\ci{.005} & .961\ci{.121} & .765\ci{.022} & .033\ci{.005} & .896\ci{.019} & .382\ci{.037} & .039\ci{.009} & .946\ci{.013} & .685\ci{.050} & 1,707 & $L^4$ \\
WCAM & .821\ci{.026} & .076\ci{.017} & .883\ci{.061} & .772\ci{.018} & .097\ci{.011} & .877\ci{.012} & .655\ci{.030}\nsd & .079\ci{.019} & .917\ci{.017} & \na & 45,939 & $L^2$ \\
\midrule
\ours{\method} & \second{.919}\ci{.026} & \best{.648}\ci{.068} & \second{.766}\ci{.095} & \second{.957}\ci{.011} & \best{.895}\ci{.025} & \best{.737}\ci{.019} & .684\ci{.031} & \second{.220}\ci{.045} & \second{.774}\ci{.027} & \best{.949}\ci{.020} & 6.3 & $k\log L$ \\


==> tables/T3_std_body.tex <==
\ctrl{Random map} & \ctrl{.152\ci{.009}} & \ctrl{.352\ci{.016}} & \ctrl{-.050\ci{.008}} & \ctrl{.090\ci{.007}} & \ctrl{.239\ci{.012}} & \ctrl{-.043\ci{.008}} & \ctrl{.250\ci{.000}} \\
\ctrl{Centre map} & \ctrl{.194\ci{.011}} & \ctrl{.576\ci{.020}} & \ctrl{.184\ci{.015}} & \ctrl{.169\ci{.009}} & \ctrl{.507\ci{.020}} & \ctrl{.172\ci{.014}} & \ctrl{.250\ci{.000}} \\
\midrule
Occlusion & .192\ci{.015} & .655\ci{.017} & .310\ci{.020} & .107\ci{.008} & .615\ci{.017} & .440\ci{.014} & .655\ci{.005} \\
RISE & .130\ci{.010} & \best{.736}\ci{.015} & .382\ci{.014} & .115\ci{.009} & \best{.675}\ci{.015} & .386\ci{.014} & .280\ci{.001} \\
LIME & .134\ci{.008} & .718\nsd\ci{.016} & .391\ci{.011} & .111\ci{.007} & .635\nsd\ci{.016} & .388\ci{.013} & .627\ci{.009} \\
KernelSHAP & .142\ci{.010} & .645\ci{.018} & .397\ci{.015} & .117\ci{.009} & .557\ci{.019} & .386\ci{.018} & \second{.846}\ci{.006} \\
PartitionSHAP & \best{.066}\ci{.005} & \second{.734}\ci{.015} & \second{.494}\ci{.012} & \second{.051}\nsd\ci{.004} & \second{.659}\ci{.016} & \second{.533}\ci{.012} & .748\ci{.011} \\
h-Shap & .332\ci{.015} & .513\ci{.019} & .118\ci{.015} & .267\ci{.014} & .433\ci{.018} & .159\ci{.015} & .797\ci{.013} \\
ShapBPT & .125\ci{.008} & .714\nsd\ci{.016} & .435\ci{.015} & .096\ci{.006} & .640\nsd\ci{.019} & .457\ci{.015} & .844\ci{.004} \\
Sobol & .111\ci{.008} & .667\ci{.018} & .455\ci{.014} & .097\ci{.007} & .582\ci{.019} & .477\ci{.014} & .686\ci{.012} \\
HSIC & .109\ci{.007} & .674\ci{.017} & .448\ci{.018} & .100\ci{.007} & .604\ci{.019} & .470\ci{.014} & .787\ci{.005} \\
LIMA & .141\ci{.009} & .675\ci{.016} & .256\ci{.012} & .115\ci{.008} & .605\ci{.018} & .287\ci{.013} & .386\ci{.004} \\
MoXI & .315\ci{.014} & .564\ci{.020} & -.050\ci{.012} & .220\ci{.012} & .508\ci{.018} & .032\ci{.012} & .309\ci{.003} \\
WCAM & .182\ci{.011} & .649\ci{.019} & .316\ci{.014} & .167\ci{.010} & .573\ci{.018} & .317\ci{.014} & .570\ci{.012} \\
\midrule
\ours{\method} & \second{.069}\ci{.006} & .717\ci{.016} & \best{.537}\ci{.012} & \best{.049}\ci{.004} & .640\ci{.017} & \best{.570}\ci{.011} & \best{.905}\ci{.006} \\


==> tables/T5_equal_body.tex <==
\tabgroup{11}{$\Delta$Pointing Game $\uparrow$}
Occlusion & .530 & .729 & .760 & .877 & .993 & .013 & .136 & .264 & .252 & .235 \\
RISE & .018 & .177 & .263 & .483 & .750 & .383 & .250 & .485 & .356 & .300 \\
Sobol & .972 & .979 & .873 & .952 & 1.000 & .233 & .205 & .319 & .356 & .500 \\
HSIC & .672 & .861 & .850 & .949 & 1.000 & .002 & .128 & .314 & .220 & .370 \\
LIME & .650 & .574 & .527 & .532 & .511 & .300 & .314 & .404 & .430 & .167 \\
KernelSHAP & .831 & .909 & .924 & .971 & .999 & .075 & .127 & .332 & .289 & .311 \\
PartitionSHAP & .770 & .854 & \na & \na & \na & .212 & .200 & \na & \na & \na \\
ShapBPT & .878 & .929 & .940 & \na & \na & .136 & .209 & .374 & \na & \na \\
HiPe & $-$.003 & .450 & .497 & .689 & .964 & $-$.010 & .076 & .140 & .135 & .210 \\
\tabgroup{11}{$\Delta$EPG $\uparrow$}
Occlusion & .550 & .720 & .758 & .849 & .948 & .065 & .061 & .071 & .051 & .114 \\
RISE & .923 & .935 & .941 & .944 & .961 & .196 & .217 & .123 & .113 & .198 \\
Sobol & .908 & .916 & .922 & .939 & .961 & .095 & .147 & .113 & .087 & .197 \\
HSIC & .830 & .881 & .886 & .923 & .952 & .117 & .099 & .114 & .096 & .141 \\
LIME & .877 & .910 & .934 & .940 & .969 & .173 & .206 & .127 & .197 & .330 \\
KernelSHAP & .793 & .855 & .865 & .914 & .952 & .028 & .060 & .082 & .091 & .156 \\
PartitionSHAP & .765 & .816 & \na & \na & \na & .057 & .035 & \na & \na & \na \\
ShapBPT & .875 & .900 & .904 & \na & \na & .093 & .094 & .114 & \na & \na \\
HiPe & .813 & .852 & .865 & .903 & .951 & .087 & .077 & .098 & .080 & .116 \\

